Deep Constrained Least Squares for Blind Image Super-Resolution

In this paper, we tackle the problem of blind image super-resolution(SR) with a reformulated degradation model and two novel modules. Following the common practices of blind SR, our method proposes to improve both the kernel estimation as well as the kernel-based high-resolution image restoration. To be more specific, we first reformulate the degradation model such that the deblurring kernel estimation can be transferred into the low-resolution space. On top of this, we introduce a dynamic deep linear filter module. Instead of learning a fixed kernel for all images, it can adaptively generate deblurring kernel weights conditional on the input and yield a more robust kernel estimation. Subsequently, a deep constrained least square filtering module is applied to generate clean features based on the reformulation and estimated kernel. The deblurred feature and the low input image feature are then fed into a dual-path structured SR network and restore the final high-resolution result. To evaluate our method, we further conduct evaluations on several benchmarks, including Gaussian8 and DIV2KRK. Our experiments demonstrate that the proposed method achieves better accuracy and visual improvements against state-of-the-art methods.

==> CVPR2022 - Super Resolution/abstract.tex <==
\begin{abstract}
%   Recent works on blind super-resolution (SR) often use PCA to project vectorized blur kernels to low dimensional linear spaces and stretch them to degradation maps with the same size as inputs. However, such a strategy destroyed the space relation of kernels and lack flexibility. Address it, we propose a new principled framework to handle the blind SR problem. Specifically, we xxx

% \vspace{-5pt}

In this paper, we tackle the problem of blind image super-resolution(SR) with a reformulated degradation model and two novel modules. Following the common practices of blind SR, our method proposes to improve both the kernel estimation as well as the kernel based high resolution image restoration. To be more specific, we first reformulate the degradation model such that the deblurring kernel estimation can be transferred into the low resolution space. On top of this, we introduce a dynamic deep linear filter module. Instead of learning a fixed kernel for all images, it can adaptively generate deblurring kernel weights conditional on the input and yields more robust kernel estimation. Subsequently, a deep constrained least square filtering module is applied to generate clean features based on the reformulation and estimated kernel. The deblurred feature and the low input image feature are then fed into a dual-path structured SR network and restore the final high resolution result. To evaluate our method, we further conduct evaluations on several benchmarks, including Gaussian8 and DIV2KRK. Our experiments demonstrate that the proposed method achieves better accuracy and visual improvements against state-of-the-art methods. 
% The source codes and pre-trained models are available at \url{https://github.com/megvii-research/DCLS-SR}. 


%In this paper, we tackle the problem of blind image super-resolution(SR) with a reformulated degradation model and two novel modules. Following the common practices of blind SR, our method consists of a kernel estimation step for deblurring and a kernel based image restoration step to recover the high resolution output. Specifically, our main improvements are three-fold: first of all, we reformulate the degradation model and propose to estimate the deblurring kernel in the low resolution space, which provides more accurate kernel estimation and a natural separation of kernel and feature learning. On top of this, we introduce a dynamic deep linear filter module. Instead of learning a fixed kernel for all images, it can adaptively generate deblurring kernel weights conditional on the input. Moreover, we propose a deep constrained least square filtering module for a better fusion of leaned kernel and features from low resolution input. Our key insight is to solve the low resolution deblurring in the feature domain and convert the filter learning into a kernel based optimization problem where the estimated kernel can be naturally integrated with input features. It also allows learning channel-wise operators w.r.t different features. The deblurred feature and the low input image feature are then fed into a dual-path based SR network and generate the final high resolution result. To evaluate our method, we further conduct evaluations on several benchmarks, including Gaussian8 and DIV2KRK. Our experiments demonstrate that the proposed method achieves better accuracy and visual improvements against state-of-the-art methods.


\end{abstract}

==> CVPR2022 - Super Resolution/conclusion.tex <==
\section{Conclusion}
In this work, we have presented a well-principled algorithm to tackle the blind SR problem. We first derive a new form of blur kernel in the low resolution space from classical degradation model. We then propose to estimate and apply that kernel in HR image restoration. Subsequently, a dynamic deep linear kernel (DDLK) module is introduced to improve kernel estimation. We further design a deep constrained least squares (DCLS) deconvolution module that integrates blur kernel and LR image in the feature domain to obtain the clean feature. The clean feature and the primitive feature are then fed into a dual-path network to generate the super-resolved image. Extensive experiments on various kernels and noises demonstrate that the proposed method leads to a state-of-the-art blind SR performance.

==> CVPR2022 - Super Resolution/experiments.tex <==
% \newpage



\section{Experiments}

\subsection{Datasets and Implementation Details}
Following previous works~\cite{gu2019blind,luo2020unfolding}, 3450 2K HR images from DIV2K~\cite{agustsson2017ntire} and Flickr2K~\cite{timofte2017ntire} are collected as the training dataset. And we synthesize corresponding LR images with specific degradation kernel settings (e.g., isotropic/anisotropic Gaussian) using Eq. ~(\ref{eq:class_degrad}). The proposed method is evaluated by PSNR and SSIM~\cite{wang2004image} on only the luminance channel of the SR results (YCbCr space).

\noindent \textbf{Isotropic Gaussian kernels.} 
Firstly, we conduct blind SR experiments on isotropic Gaussian kernels following the setting in~\cite{gu2019blind}. Specifically, the kernel sizes are fixed to 21 $\times$ 21. In training, we uniformly sample the kernel width from range [0.2, 2.0], [0.2, 3.0] and [0.2, 4.0] for SR scale factors 2, 3 and 4, respectively. For testing, we use \textit{Gaussian8}~\cite{gu2019blind} kernel setting to generate evaluation dataset from five widely used benchmarks: Set5~\cite{bevilacqua2012low}, Set14~\cite{zeyde2010single}, BSD100~\cite{martin2001database}, Urban100~\cite{huang2015single} and Manga109~\cite{matsui2017sketch}. \textit{Gaussian8} uniformly chooses 8 kernels from range [0.80, 1.60], [1.35, 2.40] and [1.80, 3.20] for scale factors 2, 3 and 4, repectively. The LR images are obtained by blurring and downsampling the HR images with selected kernels.


\noindent \textbf{Anisotropic Gaussian kernels.}
We also conduct experiments on anisotropic Gaussian kernels following the setting in~\cite{bell2019blind}. The kernel size is set to 11 $\times$ 11 and 31 $\times$ 31 for scale factors 2 and 4, respectively. During training, the anisotropic Gaussian kernels for degradation are generated by randomly selecting kernel width from range (0.6, 5) and rotating from range [-$\pi$, $\pi$]. We also apply uniform multiplicative noise and normalize it to sum to one. For evaluation, we use the DIV2KRK dataset proposed in~\cite{bell2019blind}.


\begin{figure}
\setlength{\abovecaptionskip}{0.05in}
\setlength{\belowcaptionskip}{-0.05in}
\centering
	\begin{minipage}[t]{0.49\linewidth}
		\centering
		\includegraphics[width=1.64in]{figs/compare_psnr.pdf}
	\end{minipage}
	\begin{minipage}[t]{0.49\linewidth}
		\centering
		\includegraphics[width=1.57in]{figs/compare_psnr_manga.pdf}
	\end{minipage}
	\caption{The PSNR performance curves on Set5 and Manga109 of scale factor 4. The kernel width $\sigma$ are set from 1.8 to 3.2. }
	\label{fig:cmp_psnr}
\end{figure}


\begin{figure}[t]
\setlength{\abovecaptionskip}{-0.1in}
\setlength{\belowcaptionskip}{-0.1in}
\begin{center}
\includegraphics[width=.98\linewidth]{figs/cmp_noise.pdf}
\end{center}
\caption{Visual results of \textit{Img 33} from Urban100.}
\label{fig:cmp_noise}
\end{figure}


\noindent \textbf{Implementation details.}
For all experiments, we use 5 dual-path groups, each containing 10 DPABs with 64 channels. The batch sizes are set to 64 and the LR patch sizes are 64 $\times$ 64. We use Adam~\cite{kingma2014adam} optimizer with $\beta_1=0.9$ and $\beta_2=0.99$. All models are trained on 4 RTX2080Ti GPUs with $5 \times 10^5$ iterations. The initial learning rate is set to $4 \times 10^{-4}$ and decayed by half at every $2 \times 10^{-4}$ iterations. We also augment the training data with random horizontal flips and 90 degree rotations. 


\begin{table}[t]
\setlength{\abovecaptionskip}{0.05in}
\setlength{\belowcaptionskip}{-0.05in}
\centering
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{lcccc}
\toprule
\multirow{3}{*}{Method}     & \multicolumn{4}{c}{DIV2KRK~\cite{bell2019blind}}     \\ %\cline{2-5}

& \multicolumn{2}{c}{$\times$2}              & \multicolumn{2}{c}{$\times$4}    \\ 
& PSNR  & SSIM         & PSNR  & SSIM  \\ \midrule
Bicubic & 28.73 &0.8040   &25.33 &0.6795  \\
Bicubic+ZSSR~\cite{shocher2018zero} & 29.10 &0.8215   &25.61 &0.6911  \\
EDSR~\cite{lim2017enhanced} & 29.17 &0.8216   &25.64 &0.6928  \\
RCAN~\cite{zhang2018image} & 29.20 &0.8223   &25.66 &0.6936  \\
DBPN~\cite{haris2018deep} & 29.13 & 0.8190   &25.58 &0.6910  \\
DBPN~\cite{haris2018deep}+Correction~\cite{hussein2020correction} & 30.38 &0.8717   &26.79 &0.7426  \\

KernelGAN~\cite{bell2019blind}+SRMD~\cite{zhang2018learning}  & 29.57 &0.8564   &27.51 &0.7265  \\
% KernelGAN~\cite{bell2019blind}+USRNet~\cite{zhang2020deep}  & - & -   &20.06 &0.5359  \\
KernelGAN~\cite{bell2019blind}+ZSSR~\cite{shocher2018zero}  & 30.36 & 0.8669   &26.81 &0.7316  \\

IKC~\cite{gu2019blind} & -  & -   &27.70 &0.7668  \\
DANv1~\cite{luo2020unfolding} & 32.56 & 0.8997      &27.55 &0.7582  \\
DANv2~\cite{luo2021endtoend} & {\color[HTML]{3531FF} 32.58} & {\color[HTML]{3531FF} 0.9048}     & {\color[HTML]{3531FF} 28.74} & {\color[HTML]{3531FF} 0.7893}    \\ 
AdaTarget~\cite{jo2021adatarget} & -  & -   &28.42 &0.7854  \\
KOALAnet~\cite{kim2021koalanet} & 31.89 & 0.8852     & 27.77 & 0.7637    \\ 


DCLS(Ours) & {\color[HTML]{FE0000} 32.75} & {\color[HTML]{FE0000} 0.9094}     & {\color[HTML]{FE0000} 28.99} & {\color[HTML]{FE0000} 0.7946}  \\
\bottomrule
\end{tabular}
}
\caption{Quantitative comparison on DIV2KRK. The best one marks in {\color{red}{red}} and the second best are in {\color{blue}{blue}}.}
\label{table:aniso_cmp}
\end{table}


\subsection{Comparison with State-of-the-arts}

\noindent \textbf{Evaluation with isotropic Gaussian kernels.} 
Following~\cite{gu2019blind}, we evaluate our method on datasets synthesized by \textit{Gaussian8} kernels. We compare our method with state-of-the-art blind SR approaches: ZSSR~\cite{shocher2018zero} (with bicubic kernel), IKC~\cite{gu2019blind}, DANv1~\cite{luo2020unfolding}, DANv2~\cite{luo2021endtoend} and AdaTarget~\cite{jo2021adatarget}. Following~\cite{gu2019blind}, we also conduct comparison with CARN~\cite{ahn2018fast} and its variants of performing blind deblurring method~\cite{pan2017deblurring} before and after CARN. For most methods, we use their official implementations and pre-trained models. 


\begin{figure}[t]
\setlength{\abovecaptionskip}{-0.1in}
\setlength{\belowcaptionskip}{-0.05in}
\begin{center}
\includegraphics[width=.94\linewidth]{figs/cmp_k.pdf}
\end{center}
\caption{Visual results of estimated kernels of \textit{Img 33} and \textit{Img 43} from DIV2KRK~\cite{bell2019blind} by various kernel estimation methods.}
\label{fig:cmp_k}
\end{figure}

\begin{table}[t]
\setlength{\abovecaptionskip}{0.05in}
\setlength{\belowcaptionskip}{-0.1in}
\centering
\resizebox{.95\linewidth}{!}{
\begin{tabular}{ccccc}
\toprule
DIV2KRK $\times4$   & KernelGAN   & CorrFilter      & DANv2  & DDLK       \\ \midrule

% K-PSNR      &56.65        & 58.92       & 66.95   & 67.13     \\
LR-PSNR $\uparrow$      &41.28      & 41.35      & 45.06      & \textbf{45.27}   \\
Kernel-MSE $\downarrow$     & 0.1518    & 0.1392       & 0.0817   & \textbf{0.0574}   \\


\bottomrule
\end{tabular}
}
\caption{Quantitative evaluation on the performance of DDLK.}
\label{table:cmp_k}
\end{table}


\begin{figure*}[t]
\setlength{\abovecaptionskip}{-0.1in}
\setlength{\belowcaptionskip}{-0.1in}
\begin{center}
\includegraphics[width=.999\linewidth]{figs/cmp_iso.pdf}
\end{center}
\caption{Visual results of \textit{Img 67} and \textit{Img 73} in Urban100~\cite{huang2015single}, for scale factor 4 and kernel width 2.6. Best viewed in color.}
\label{fig:cmp_iso}
\end{figure*}


\begin{figure*}[t]
\setlength{\abovecaptionskip}{-0.1in}
\setlength{\belowcaptionskip}{-0.1in}
\begin{center}
\includegraphics[width=.999\linewidth]{figs/cmp_aniso.pdf}
\end{center}
\caption{Visual results of \textit{Img 36} and \textit{Img 12} in DIV2KRK~\cite{bell2019blind}, for scale factor of 4. Best viewed in color.}
\label{fig:cmp_aniso}
\end{figure*}

The quantitative results are shown in \Cref{table:iso_cmp}. It is obvious that our method leads to the best performance over all datasets. The bicubic SR model CARN suffers severe performance drop with \textit{Gaussian8} which deviates from the predefined bicubic kernel. Performing deblurring on the super-resolved image can improve the results. ZSSR achieves better performance compared with non-blind SR method but is limited by the image-specific network design (cannot utilize abundant training data). AdaTarget can improve image quality but is still inferior to that of blind SR methods. IKC and DAN are two-step blind SR methods and can largely improve the results. However, both of them predict kernel embedding and directly involve it into the network, which damages the spatial relation of the kernel and thus performs inferior to our method. We also provide the comparison of PSNR values on different datasets with blur kernels width from 1.8 to 3.2 as shown in Fig.~\ref{fig:cmp_psnr}. DCLS performs the best result over all different kernel widths. The qualitative results shown in Fig.~\ref{fig:cmp_iso} illustrate that DCLS can produce clear and pleasant SR images. Furthermore, we conduct an experiment of super-resolving images with additional noise. As shown in~\Cref{table:iso_noise_cmp} and Fig.~\ref{fig:cmp_noise}, DCLS still outperforms other methods over all datasets with different noise levels.



\noindent \textbf{Evaluation with anisotropic Gaussian kernels.} 
Degradation with anisotropic Gaussian kernels are more general and challenging. Similar to isotropic kernel, we firstly compare our method with SOTA blind SR approaches such as ZSSR~\cite{shocher2018zero}, IKC~\cite{gu2019blind}, DANv1~\cite{luo2020unfolding}, DANv2~\cite{luo2021endtoend}, AdaTarget~\cite{jo2021adatarget} and KOALAnet~\cite{kim2021koalanet}. We also compare DCLS with some SOTA bicubicly designed methods such as EDSR~\cite{lim2017enhanced}, RCAN~\cite{zhang2018image}, and DBPN~\cite{haris2018deep}. And we provide Correction~\cite{hussein2020correction} for DBPN. In addition, we combine a kernel estimation method (e.g. KernelGAN~\cite{bell2019blind}) with other non-blind SR methods, such as ZSSR~\cite{shocher2018zero} and SRMD~\cite{zhang2018learning}, as two-step solutions to solve blind SR. 

Table~\ref{table:aniso_cmp} shows the quantitative results on DIV2KRK~\cite{bell2019blind}. It can be seen that the proposed DCLS significantly improves the performance compared with other blind SR approaches. Note that ZSSR performs better when combined with KernelGAN, which indicates that good kernel estimation can help a lot. Recent SOTA blind SR methods such as IKC, DAN and KOALAnet can achieve remarkable accuracy in PSNR and SSIM. By applying an adaptive target to finetune the network, AdaTarget can perform comparably with SOTA blind methods. However, all of those methods are still inferior to the proposed DCLS. The visual results on DIV2KRK are shown in \cref{fig:cmp_aniso}. As we can see, the SR images produced by our method are much sharper and cleaner. We also provide the results of kernel estimation and downsampling HR image with estimated kernel in Fig.~\ref{fig:cmp_k} and Table~\ref{table:cmp_k}. Compared with previous image-specific methods such as KernelGAN~\cite{bell2019blind} and Correction Filter~\cite{hussein2020correction}, the dynamic deep linear kernel (DDLK) is more flexible and capable of producing accurate kernels.



\subsection{Analysis and Discussions}

\begin{table}[t]
\setlength{\abovecaptionskip}{0.05in}
\setlength{\belowcaptionskip}{-0.1in}
\centering
\resizebox{1.\linewidth}{!}{
\begin{tabular}{ccccc|cc}
\toprule
 \multirow{2}{*}{SLK}     & \multirow{2}{*}{DDLK}  & \multirow{2}{*}{\tabincell{c}{Stretching \\ Strategy}}   & \multirow{2}{*}{\tabincell{c}{DCLS \\ Deconv}}   & \multirow{2}{*}{DPAN}   & \multicolumn{2}{c}{DIV2KRK}     \\

    &      &     &      &   & PSNR  & SSIM    \\  \hline

 $\checkmark$     & -  & $\checkmark$     & -  & $\checkmark$  & 28.84 & 0.7921 \\
 -     & $\checkmark$       & $\checkmark$     &-  & $\checkmark$  & 28.86 & 0.7924    \\
$\checkmark$    & -       & -     & $\checkmark$  & $\checkmark$  & 28.94 & 0.7946    \\
 -     & $\checkmark$       & -    & $\checkmark$   & -  & 28.94 & 0.7938    \\
 -     & $\checkmark$       & -    & $\checkmark$   & $\checkmark$  & 28.99 & 0.7964    \\

\bottomrule
\end{tabular}
}
\caption{Ablation study on our vital components.}
\label{table:ablation}
\end{table}



% \begin{table}[t]
% \centering
% \resizebox{1.\linewidth}{!}{
% \begin{tabular}{ccccccc}
% \toprule
% \multirow{2}{*}{Method}    & \multicolumn{2}{c}{Set14}       & \multicolumn{2}{c}{Urban100}       & \multicolumn{2}{c}{DIV2KRK}     \\
%   & PSNR & SSIM     & PSNR & SSIM   & PSNR & SSIM   \\ \midrule
% $\rm Winner_{Fea}$      & 28.38 & 0.7709     & 26.07 & 0.7775     & 28.88 & 0.7936    \\  
% $\rm CLS_{Fea}$     & 28.29 & 0.7658    & 26.04 & 0.7768     & 28.92 & 0.7921    \\
% $\rm DCLS_{Fea}$    & 28.54 & 0.7728   & 26.15 & 0.7809     & 28.99 & 0.7946    \\

% \bottomrule
% \end{tabular}
% }
% \caption{Quantitative comparison on various datasets. $\rm Fea$ means applying deconvolution on the feature space.}
% \label{table:fea-deconv}
% \end{table}


\begin{table}[t]
\setlength{\abovecaptionskip}{0.05in}
\setlength{\belowcaptionskip}{-0.08in}
\centering
\resizebox{1.\linewidth}{!}{
\begin{tabular}{lcccccc}
\toprule
\multirow{2}{*}{Method}    & \multicolumn{2}{c}{$\rm Wiener_{Fea}$~\cite{dong2020deep}}       & \multicolumn{2}{c}{$\rm CLS_{Fea}$}       & \multicolumn{2}{c}{$\rm DCLS_{Fea}$}     \\
  & PSNR & SSIM     & PSNR & SSIM   & PSNR & SSIM   \\ \midrule
Set5      & 32.05 & 0.8878     & 31.98 & 0.8862     & \textbf{32.12} & \textbf{0.8890}    \\  
Set14     & 28.38 & 0.7709    & 28.29 & 0.7658     & \textbf{28.54} & \textbf{0.7728}    \\
BSD100    & 27.47 & 0.7238   & 27.48 & 0.7216     & \textbf{27.60} & \textbf{0.7285}    \\
Urban100    & 26.07 & 0.7775   & 26.03 & 0.7768     &\textbf{26.15} & \textbf{0.7809}    \\
Manga109    & 30.77 & 0.9069   & 30.65 & 0.9040     &\textbf{30.86} & \textbf{0.9086}    \\
DIV2KRK    & 28.77 & 0.7886   & 28.92 & 0.7921     &\textbf{28.99} & \textbf{0.7947}    \\

\bottomrule
\end{tabular}
}
\caption{Quantitative comparison on various datasets. $\rm Fea$ means applying deconvolution on the feature space.}
\label{table:fea-deconv}
\end{table}

\begin{table}[t]
\setlength{\abovecaptionskip}{0.05in}
\setlength{\belowcaptionskip}{-0.1in}
\centering
\resizebox{.99\linewidth}{!}{
\begin{tabular}{ccccc}
\toprule
DIV2KRK $\times$4    & $\rm Wiener_{RGB}$   & $\rm CLS_{RGB}$      & $\rm DCLS_{RGB}$  & $\rm DCLS_{Fea}$       \\ \midrule

PSNR      & 28.91     &28.90      & 28.94       & 28.99     \\
SSIM      & 0.7941    &0.7935     & 0.7941      & 0.7964      \\

\bottomrule
\end{tabular}
}
\caption{Quantitative results. $\rm RGB$ and $\rm Fea$ mean applying deconvolution in the RGB space and feature space, respectively.}
\label{table:rgb-deconv}
\end{table}


\noindent \textbf{Ablation Study.} 
We conduct ablation studies on vital components of our method: DPAN, DDLK and DCLS deconvolution. 
% The baseline model uses DPAN architecture and estimates a single layer kernel (SLK), and adopts the kernel stretching strategy following~\cite{gu2019blind,luo2020unfolding}. 
The quantitative results on DIV2KRK are exported in \Cref{table:ablation}. Note that the baseline model with DPAN eliminates artifacts from kernel and thus improves the result. And the DCLS deconvolution can further make use of the estimated kernel and high-level information from deep features to achieve a higher performance (+0.15dB from baseline). 
% Obviously, we can benefit from DDLK and DCLS deconvolution. 

\noindent \textbf{Effectiveness of the DCLS deconvolution.} 
To illustrate the effectiveness of DCLS, we include a comparison of substituting DCLS with other deblurring methods, such as traditional constrained least squares (CLS) and Wiener deconvolution~\cite{wiener1964extrapolation,dong2020deep} in the RGB space and feature space. The results are presented in Table~\ref{table:fea-deconv} and Table~\ref{table:rgb-deconv}. By applying deconvolution in the RGB space with the reformulated kernel, we can get a clear LR image and thus improve the SR performance. This idea is similar to Correction Filter~\cite{hussein2020correction}, but with one big difference, in that our estimator is highly correlated to the LR image rather than the SR model. The visual example is shown in Fig.~\ref{fig:dcls_rgb}.

\noindent \textbf{Performance on Real Degradation} 
To further demonstrate the effectiveness of our method, we apply the proposed model on real degradation data where the ground truth HR images and the blur kernels are not available. An example of super-resolving historic image is shown in Fig.~\ref{fig:realim}. Compared with LapSRN~\cite{lai2017deep} and DANv2~\cite{luo2021endtoend}, our DCLS can produce sharper edges and visual pleasing SR results.

\begin{figure}[t]
\setlength{\abovecaptionskip}{-0.1in}
\setlength{\belowcaptionskip}{-0.05in}
\begin{center}
\includegraphics[width=1.\linewidth]{figs/deblur_rgb4.pdf}
\end{center}
\caption{Applying DCLS in the RGB space. (a) Original LR \& kernel, (b) corrected LR \& estimated kernel by~\cite{hussein2020correction}, (c) deblurred LR \& estimated kernel by the proposed method.}
\label{fig:dcls_rgb}
\end{figure}


% \begin{figure}[t]
% % \setlength{\abovecaptionskip}{-0.in}
% % \setlength{\belowcaptionskip}{0.in}
% \begin{center}
% \includegraphics[width=.9\linewidth]{figs/compare_psnr.pdf}
% \end{center}
% \caption{The PSNR performance of different methods on Set5 of scale factor is 4. The kernel width $\sigma$ are set from 1.8 to 3.2. }
% \label{fig:set5_psnr}
% \end{figure}

% \begin{figure}[t]
% % \setlength{\abovecaptionskip}{-0.in}
% % \setlength{\belowcaptionskip}{0.in}
% \begin{center}
% \includegraphics[width=.9\linewidth]{figs/compare_psnr_manga.pdf}
% \end{center}
% \caption{The PSNR performance of different methods on Manga109 of scale factor is 4. The kernel width $\sigma$ are set from 1.8 to 3.2. }
% \label{fig:manga_psnr}
% \end{figure}

\begin{figure}[t]
\setlength{\abovecaptionskip}{-0.1in}
\setlength{\belowcaptionskip}{-0.1in}
\begin{center}
\includegraphics[width=1.\linewidth]{figs/realim.pdf}
\end{center}
\caption{Comparison of historic image~\cite{lai2017deep} for 4$\times$ SR.}
\label{fig:realim}
\end{figure}



==> CVPR2022 - Super Resolution/introduction.tex <==


% \begin{figure*}[t]
% \setlength{\abovecaptionskip}{-0.in}
% % \setlength{\belowcaptionskip}{0.in}
% \begin{center}
% \includegraphics[width=1.\linewidth]{figs/ts.pdf}
% \end{center}
% \caption{Blind super-resolution of \textit{Img 28} from DIV2KRK, for scale factor 4. The proposed method outperforms previous state-of-the-art approaches such as KernelGAN~\cite{bell2019blind}+ZSSR~\cite{shocher2018zero}, IKC~\cite{gu2019blind}, DAN~\cite{luo2020unfolding,luo2021endtoend}, AdaTarget~\cite{jo2021adatarget}, and KOALAnet~\cite{kim2021koalanet}.}
% \label{fig:ts}
% \end{figure*}

\section{Introduction}
In this work, we study the problem of image super-resolution,i.e., restoring high-resolution images from low-resolution inputs. Specially, we aim for single image super-resolution (SISR), where only one observation is given which is a more practical setting and with a wide range of downstream applications ~\cite{dong2014learning,kim2016accurate,lim2017enhanced,ledig2017photo,zhang2018image,wang2018esrgan,fritsche2019frequency,li2019feedback,zhang2019deep,haris2018deep}.   

Most existing works based on the classical SISR degradation model assuming that the input LR image ${\bf y}$ is a blurred and down-scaled HR image ${\bf x}$ with additional white Gaussian noise {\bf n}, given by
\begin{equation}
\centering
    {\bf y} = ({\bf x} \ast {\bf k}_h)_{\downarrow_s} + {\bf n},
\label{eq:class_degrad}
\end{equation}
where ${\bf k}_h$ is the blur kernel applied on $\bf x$, $\ast$ denotes convolution operation and $\downarrow_s$ denotes downsampling with scale factor $s$. 
% \paragraph{issue with this model}
Previous blind SR approaches ~\cite{gu2019blind,luo2020unfolding} generally solve this problem with a two-stage framework: kernel estimation from LR image and kernel based HR image restoration. 

We argue that although such a pipeline demonstrates reasonable performance for SR problem, there are two main drawbacks: First of all, it is difficult to accurately estimate blur kernels of HR space directly from LR images due to the ambiguity produced by undersampling step ~\cite{vandewalle2006frequency,park2003super}. And the mismatch between the estimated kernel and the real one will cause significant performance drop and even lead to unpleasant artifacts~\cite{zhang2018learning,gu2019blind,bell2019blind,hussein2020correction}.
% for networks that are sensitive to these kernels 
Secondly, it is also challenging to find a suitable way to fully utilize the information of the estimated HR space kernel and LR space image. A common solution is to employ a kernel stretching strategy ~\cite{zhang2018learning,gu2019blind,luo2020unfolding}, where the principal components of the vectorized kernel are preserved and stretched into degradation maps with the same size as the LR input. These degradation maps then can be concatenated with the input image or its features to generate a clean HR image. However, the spatial relation of the kernel is destroyed by the process of vectorizing and PCA (Principal Component Analysis), which causes insufficient usage of the kernel.  The subsequent reconstruction network requires a huge effort to harmonize the inconsistent information between LR features and HR-specific kernels, limiting its performance in super-resolving images.


%Blind SR approaches solve this problem by firstly estimating a kernel from LR image, and then recover the HR image based on that kernel. Recent studies~\cite{zhang2018learning,gu2019blind,bell2019blind,hussein2020correction} show that networks are sensitive to these kernels and often suffer performance drop and even produce unpleasant artifacts when the estimated kernel is mismatch the real one. However, the aliasing ambiguity produced from undersampling~\cite{vandewalle2006frequency,park2003super} makes it difficult to accurately estimate such kernel from low-resolution space. 
% Although several works have made efforts in kernel estimation, 

%On the other hand, to recover the HR image from LR input and the corresponding kernel, the common solution is to employ a kernel stretching strategy~\cite{zhang2018learning,gu2019blind,luo2020unfolding}, where the principal components of the vectorized kernel are preserved and stretched into degradation maps which are the same size as the LR input. By doing so, these degradation maps can be concatenated with input image or its feature to generate clean HR image. However, the spatial relation of kernel is destroyed by the process of vectorizing and PCA (Principal Component Analysis), which causes insufficient usage of the kernel. Moreover, since the kernel ${\bf k}_h$ is primitively applied on the HR image, concatenating it with LR as input is implausible. The subsequent reconstruction network requires a huge effort to harmonize the inconsistent information between LR features and HR-specific kernels, limiting its performance in super-resolving images.

% \paragraph{our method}

%In this paper, we present a different strategy to tackle the blind SR problem which can naturally avoid the above motioned drawbacks. Specifically, we reformulate the degradation model to apply another kernel ${\bf k}_l$ in the downsampled low-resolution space so that the kernel estimating can be free of aliasing. To be consistent with classical degradation, the kernel ${\bf k}_l$ in the new formulation is derived from the primitive kernel ${\bf k}_h$ and HR image.  Based on such the new degradation model, we further introduce the dynamic deep linear kernel (DDLK). Compared with estimating a single layer kernel, DDLK can provide more equivalent choices of possible optimal solutions for the kernel, which is easier to optimize. Since no nonlinear layer is used, DDLK can be analytically collapsed to a single layer kernel. Moreover, we propose a deep constrained least squares (DCLS) deconvolution module applied to the deep feature domain so as to obtain deblurred features to restore a super-resolved clean image. 


Towards this end, we present a modified learning strategy to tackle the blind SR problem, which can naturally avoid the above mentioned drawbacks. Specifically, we first reformulate the degradation model in a way such that the blur kernel estimation and image upsampling can be disentangled. In particular, as shown in Fig.~\ref{fig:reform_kernels}, we derive a new kernel from the primitive kernel ${\bf k}_h$ and LR image. It transfers the kernel estimation into the LR space and the new kernel can be estimated without aliasing ambiguity. Based on the new degradation, we further introduce the dynamic deep linear kernel (DDLK) to provide more equivalent choices of possible optimal solutions for the kernel to accelerate training. 
% Since no nonlinear layer is used, DDLK can be analytically collapsed to a single layer kernel. 
Subsequently, a novel deep constrained least squares (DCLS) deconvolution module is applied in the feature domain to obtain deblurred features. DCLS is robust to noise and can provide a theoretical and principled guidance to obtain clean images/features from blurred inputs. Moreover, it dosen't require kernel stretching strategy and thus preserves the kernel's spatial relation information. Then the deblurred features are fed into an upsampling module to restore the clean HR images. As illustrated in Fig.~\ref{fig:ts}, the overall method has turned out to be surprisingly effective in recovering sharp and clean SR images.

% To evaluate our method, we conduct experiments in several benchmarks, including DIV2KRK~\cite{bell2019blind} and \textit{Gaussian8}~\cite{gu2019blind}. The latter is generated by applying 8 isotropic Gaussian kernels on commonly used datasets such as Set5~\cite{bevilacqua2012low}, Set14~\cite{zeyde2010single}, BSD100~\cite{martin2001database}, Urban100~\cite{huang2015single} and Manga109~\cite{matsui2017sketch}.

% \paragraph{experiments}
The main contributions are summarized as follows:

\begin{itemize}
    \item We introduce a new practical degradation model derived from \cref{eq:class_degrad}. Such degradation maintains consistency with the classical model and allows us reliably estimate blur kernel from low-resolution space.
    
    \item We propose to use a dynamic deep linear kernel instead of a single layer kernel, which provides more equivalent choices of the optimal solution of the kernel, which is easier to learn.
    
    \item We propose a novel deconvolution module named DCLS that is applied on the features as channel-wise deblurring so that we can obtain a clean HR image.
    
    \item Extensive experiments on various degradation kernels demonstrate that our method leads to state-of-the-art performance in blind SR problems.
\end{itemize}

\vspace{-0.1in}

\begin{figure}[t]
\setlength{\abovecaptionskip}{-0.05in}
\setlength{\belowcaptionskip}{-0.1in}
\begin{center}
% \includegraphics[width=1.0\linewidth]{figs/deep_linear_kernel.pdf}
\includegraphics[width=.99\linewidth]{figs/reform_kernels.pdf}
\end{center}
\caption{Kernel reformulation examples. The top row and middle row are the LR images and the corresponding primitive kernels. The bottom row is the reformulated kernels.}
\label{fig:reform_kernels}
\end{figure}


==> CVPR2022 - Super Resolution/method.tex <==
% \newpage



\section{Method}
We now formally introduce our method which consists of three main components given a reformation of degradation: A dynamic deep linear kernel estimation module and a deep constrained least squares module for kernel estimation and LR space feature based deblur. A dual-path network is followed to generate the clean HR output. We will first derive the reformulation and then detail each module.  


\subsection{Degradation Model Reformulation}


% To explicitly embed the deconvolution module at the low-resolution space, 
Ideally, the blur kernel to be estimated and its corresponding image should be in the same low-resolution space such that the degradation can be transformed to the deblurring problem followed by a SISR problem with bicubic degradation~\cite{zhang2018learning,zhang2019deep}.
Towards this end, we propose to reformulate Eq.~(\ref{eq:class_degrad}) as
\begin{align}
\centering
    {\bf y} &= {\cal F}^{-1}\left({\cal F}\left(({\bf x} \ast {\bf k}_h)_{\downarrow_s}\right)\right) + {\bf n}\\
            &= {\cal F}^{-1}\left({\cal F}\left({\bf x}_{\downarrow_s}\right)\frac{{\cal F}\left(({\bf x} \ast {\bf k}_h)_{\downarrow_s}\right)}{{\cal F}\left({\bf x}_{\downarrow_s}\right)} \right) + {\bf n} \\
            &= {\bf x}_{\downarrow_s} \ast {\cal F}^{-1}\left(\frac{{\cal F}\left(({\bf x} \ast {\bf k}_h)_{\downarrow_s}\right)}{{\cal F}\left({\bf x}_{\downarrow_s}\right)} \right) + {\bf n},
\label{eq:derive_new_degrad}
\end{align}
where $\cal F$ denotes the Discrete Fourier Transform and ${\cal F}^{-1}$ denotes its inverse. Then let
\begin{equation}
\centering
    {\bf k}_l = {\cal F}^{-1}\left(\frac{{\cal F}\left(({\bf x} \ast {\bf k}_h)_{\downarrow_s}\right)}{{\cal F}\left({\bf x}_{\downarrow_s}\right)}\right),
\label{eq:derive_k}
\end{equation}
we can obtain another form of degradation:
\begin{equation}
\centering
    {\bf y} = {\bf x}_{\downarrow_s} \ast {\bf k}_l + {\bf n}.
\label{eq:new_degrad}
\end{equation}
In the \cref{eq:new_degrad}, ${\bf k}_l$ is derived from the corresponding ${\bf k}_h$ and applied on the downsampled HR image ${\bf x}_{\downarrow_s}$. 
% Assuming the noise $\bf n$ is independent from the clear ${\bf x}$ and ${\bf x}\downarrow_s$, we can derive that
% \begin{equation}
% \centering
%     {\bf x}_{\downarrow_s} \ast {\bf k}_l = ({\bf x} \ast {\bf k}_h)_{\downarrow_s}.
% \end{equation}
% Then we can obtain ${\bf k}_l$ based on original blur kernel ${\bf k}_h$ and HR image $\bf x$ as
% \begin{equation}
% \centering
%     {\bf k}_l = {\cal F}^{-1}\left(\frac{{\cal F}\left(({\bf x} \ast {\bf k}_h)_{\downarrow_s}\right)}{{\cal F}\left({\bf x}_{\downarrow_s}\right)}\right),
% \label{eq:derive_k}
% \end{equation}
% where $\cal F$ denotes the Discrete Fourier Transform and ${\cal F}^{-1}$ denotes its inverse. 
To ensure numerical stability, we rewrite Eq.~(\ref{eq:derive_k}) with a small regularization parameter $\epsilon$:
\begin{equation}
\centering
    {\bf k}_l = {\cal F}^{-1}\left(\frac{\overline{{\cal F}({\bf x}_{\downarrow_s})}}{\overline{{\cal F}({\bf x}_{\downarrow_s})}{\cal F}({\bf x}_{\downarrow_s}) + \epsilon} {\cal F}\left(({\bf x} \ast {\bf k}_h)_{\downarrow_s}\right)\right),
\label{eq:derive_stable_k}
\end{equation}
where $\overline{{\cal F}(\cdot)}$ is the complex conjugate of ${\cal F}$. Fig.~\ref{fig:reform_kernels} illustrates the results of reformulating kernels by \cref{eq:derive_stable_k}. Based on the new degradation process, our goal is to estimate the blur kernel ${\bf k}_l$ and then restore HR image $\bf x$.

% \begin{figure}[t]
% \setlength{\abovecaptionskip}{-0.05in}
% \setlength{\belowcaptionskip}{-0.1in}
% \begin{center}
% % \includegraphics[width=1.0\linewidth]{figs/deep_linear_kernel.pdf}
% \includegraphics[width=.99\linewidth]{figs/reform_kernels.pdf}
% \end{center}
% \caption{Visual examples of reformulating kernel by \cref{eq:derive_stable_k}. The top row and middle row are the LR images and the corresponding primitive kernels from DIV2KRK. The bottom row is reformulated kernels as ${\bf k}_l$ in \cref{eq:new_degrad}.}
% \label{fig:reform_kernels}
% \end{figure}

\begin{figure}[t]
\setlength{\abovecaptionskip}{-0.in}
\setlength{\belowcaptionskip}{-0.1in}
\begin{center}
% \includegraphics[width=1.0\linewidth]{figs/deep_linear_kernel.pdf}
\includegraphics[width=.9\linewidth]{figs/ddlk.pdf}
\end{center}
\caption{Architecture of the dynamic deep linear kernel.}
\label{fig:DDLK}
\end{figure}

\subsection{Dynamic Deep Linear Kernel}

%Kernel estimation is a vital step in blind SR due to kernel mismatch will usually cause serve performance drop~\cite{gu2019blind,luo2020unfolding}. However, there is only one correct solution if we directly estimate a single layer kernel (all weights of estimated kernel equal to the ground-truth kernel), which is difficult due to the highly non-convex of the blind SR problem~\cite{bell2019blind}. Address it, we propose a image-specific dynamic deep linear kernel (DDLK) which consists of a sequence of linear convolution layers without activations. Theoretically, deep linear networks have infinitely equivalent global minimas~\cite{saxe2013exact,kawaguchi2016deep,bell2019blind}, which allow us to find many different filter parameters to achieve the same correct solution. Moreover, since no non-linearity is used in the network, we can analytically collapse a deep linear kernel as a single layer kernel.

Following the reformation, we start our blind SR method from the kernel estimation. A straightforward solution is to adopt a regression network to estimate kernel ${\bf \hat k}$ by minimizing the L1 difference w.r.t the new ground-truth blur kernel ${\bf k}_l$ in Eq.~(\ref{eq:derive_stable_k}). We argue such a single layer kernel (all weights of estimated kernel equal to the ground-truth kernel) estimation is in general difficult and unstable due to the highly non-convex of the blind SR problem~\cite{bell2019blind}, leading to kernel mismatch and performance drop~\cite{gu2019blind,luo2020unfolding}. Instead, we propose an image-specific dynamic deep linear kernel (DDLK) which consists of a sequence of linear convolution layers without activations. Theoretically, deep linear networks have infinitely equivalent global minimas~\cite{saxe2013exact,kawaguchi2016deep,bell2019blind}, which allow us to find many different filter parameters to achieve the same correct solution. Moreover, since no non-linearity is used in the network, we can analytically collapse a deep linear kernel as a single layer kernel.


\begin{figure*}[t]
\setlength{\abovecaptionskip}{-0.in}
\setlength{\belowcaptionskip}{0.in}
\begin{center}
\includegraphics[width=1.\linewidth]{figs/pipeline3.pdf}
\end{center}
\caption{The overview architecture of the proposed method. Given an LR image $\bf y$, we first estimate the degradation kernel $\hat{\bf k}$, and involve it in the deep constrained least squares (DCLS) convolution in the feature domain. The deblurred features $\widehat {\cal R}$ are then concatenated with primitive features ${\cal G}{\bf y}$ to restore the clean HR image $\bf x$ through a dual-path attention network (DPAN).}
\label{fig:pipline}
\end{figure*}

Fig.~\ref{fig:DDLK} depicts an example of estimating 4 layers dynamic deep linear kernel. The filters are set to $11\times11$, $7\times7$, $5\times5$ and $1\times1$, which make the receptive field to be $21\times21$. We first generate the filters of each layer based on the LR image, and explicitly sequentially convolve all filters into a single narrow kernel with stride 1. Mathematically, let ${\bf h}_i$ represent the $i$-th layer filter, we can get a single layer kernel following
\begin{equation}
\centering
    {\bf \hat k} = {\bf I_k} \ast {\bf h}_1 \ast {\bf h}_2 \ast \cdots \ast  {\bf h}_r
\label{eq:convolve_k}
\end{equation}
where $r$ is the number of linear layers, ${\bf I_k}$ is an identity kernel. As an empirically prior, we also constrain the kernel ${\bf \hat k}$ sum up to 1. The kernel estimation network can be optimized by minimizing the L1 loss between estimated kernel ${\bf \hat k}$ and new ground-truth blur kernel ${\bf k}_l$ from Eq.~(\ref{eq:derive_stable_k}).
% \begin{equation}
% \centering
%     {\cal L}_k = \frac{1}{N} \sum_{i=1}^N \left \Vert {\bf \hat k} - {\bf k}_l \right \Vert_1
% \label{eq:k_loss}
% \end{equation}


\subsection{Deep Constrained Least Squares}

Our goal is to restore HR image based on LR image and estimated kernel ${\bf \hat k}$ according to the new degradation model (Eq. (\ref{eq:new_degrad})). 
Considering a group of feature extracting linear layers $\{{\cal G}_i\}_{i=1}^L$ provided to the LR image, we can rewrite Eq. (\ref{eq:new_degrad}) in the feature space, given by
\begin{equation}
\centering
    {\cal G}_i{\bf y} = {\bf \hat k} {\cal G}_i{\bf x}_{\downarrow_s} + {\cal G}_i{\bf n}.
\label{eq:fea_degrad}
\end{equation}
Let ${\widehat {\cal R}_i}$ be the sought after deblurred feature corresponding to ${\cal G}_i{\bf x}_{\downarrow_s}$. To solve Eq. (\ref{eq:fea_degrad}), we minimize the following criterion function
\begin{equation}
\centering
    {\cal C} = || \nabla \widehat{\mathcal R}_i ||^2, \; s.t. \ \ || {\cal G}_i{\bf y} - {\bf \hat k}{\widehat {\cal R}_i} ||^2 = || {\cal G}_i{\bf n} ||^2
\label{eq:cri_func}
\end{equation}
% subject to the constraint
% \begin{equation}
% \centering
%     \left \Vert {\cal G}_i{\bf y} - {\bf \hat k}{\widehat {\cal R}_i} \right \Vert^2 = \left \Vert {\cal G}_i{\bf n} \right \Vert^2,
% \label{eq:cri_constraint}
% \end{equation}
where the $\nabla$ is a smooth filter which can be denoted by $\bf P$. Then we introduce the Lagrange function, defined by
\begin{equation}
\centering
    \min_{{\widehat {\cal R}_i}} \left [ || {\bf P} \widehat{\mathcal R}_i ||^2 + \lambda \left ( || {\cal G}_i{\bf y} - {\bf \hat k}{\widehat {\cal R}_i} ||^2 - || {\cal G}_i{\bf n} ||^2 \right) \right],
\label{eq:lagrange_func}
\end{equation}
where $\lambda$ is the Lagrange multiplier. Computing the derivative of Eq.~(\ref{eq:lagrange_func}) with respect to ${\widehat {\cal R}_i}$ and setting it to zero:
\begin{equation}
\centering
    \left( \lambda {\bf \hat k}^{\mathsf{T}}{\bf \hat k} + {\bf P}^{\mathsf{T}}{\bf P} \right) \widehat{\mathcal R}_i - \lambda {\bf \hat k}^{\mathsf{T}} {\cal G}_i{\bf y} = 0.
\label{eq:lagrange_derive}
\end{equation}
We can obtain the clear features as
\begin{equation}
\centering
    \widehat{\mathcal R}_i = {\cal H} {\cal G}_i{\bf y}.
\label{eq:dcls}
\end{equation}
where ${\cal H}_i$ denotes the deep constrained least squares deconvolution (DCLS) operator, given by
\begin{equation}
\centering
    {\cal H} = {\cal F}^{-1} \left( \frac{\overline{{\cal F}({\bf \hat k})}}{\overline{{\cal F}({\bf \hat k})}{\cal F}({\bf \hat k}) + \frac{1}{\lambda }\overline{{\cal F}({\bf P})}{\cal F}({\bf P})} \right).
\label{eq:h_simple}
\end{equation}
Different from in the standard image space (e.g. RGB), smooth filter ${\bf P}$ and variable $\lambda$ in Eq.~(\ref{eq:h_simple}) might be inconsistent in the feature space. Alternatively, we predict a group of smooth filters with implicit Lagrange multiplier for different channels through a neural network $\cal P$:
\begin{equation}
\centering
    \{\tilde {\bf P}_i\}_{i=1}^L=\{{\cal P}({\cal G}_i{\bf y})\}_{i=1}^L.
\label{eq:pred_P}
\end{equation}
% $\{\tilde {\bf P}_i\}_{i=1}^L=\{CNN({\cal G}_i{\bf y})\}_{i=1}^L$. 
Then the feature-specific operator ${\cal H}_i$ can be define by 
\begin{equation}
\centering
    {\cal H}_i = {\cal F}^{-1} \left( \frac{\overline{{\cal F}({\bf \hat k})}}{\overline{{\cal F}({\bf \hat k})}{\cal F}({\bf \hat k}) + \overline{{\cal F}(\tilde{\bf P}_i)}{\cal F}(\tilde{\bf P}_i)} \right).
\label{eq:h_deep}
\end{equation}
Now we can obtain the clear features by Eq.~(\ref{eq:dcls}) and Eq.~(\ref{eq:h_deep}). 

It is worth to note that a deep neural network (DNN) can be locally linear~\cite{dong2020deep,lee2018towards,montufar2014number}, thus we could apply DNN as ${\cal G}_i$ to extract useful features in Eq.~(\ref{eq:fea_degrad}). In addition, the consequent artifacts or errors can be compensated by the following dual-path attention module.


% \begin{figure}[t]
% % \setlength{\abovecaptionskip}{-0.in}
% % \setlength{\belowcaptionskip}{0.in}
% \begin{center}
% \includegraphics[width=.7\linewidth]{figs/dpab.pdf}
% \end{center}
% \caption{Details of the dual-path attention block. $\widehat{\mathcal R}$ and ${\cal G}{\bf y}$ are the deconvolved features and original LR features, respectively. CA represents the channel attention layer.}
% \label{fig:DPAB}
% \end{figure}



% {\color[HTML]{3531FF} 0.041} blue
% {\color[HTML]{FE0000} 37.60} red

\begin{table*}[ht]
\setlength{\abovecaptionskip}{0.05in}
\setlength{\belowcaptionskip}{-0.1in}
\centering
\resizebox{0.91\linewidth}{!}{
\begin{tabular}{cccccccccccc}
\toprule
\multirow{2}{*}{Method}& \multirow{2}{*}{Scale} & \multicolumn{2}{c}{Set5~\cite{bevilacqua2012low}}              & \multicolumn{2}{c}{Set14~\cite{zeyde2010single}}     & \multicolumn{2}{c}{BSD100~\cite{martin2001database}}      & \multicolumn{2}{c}{Urban100~\cite{huang2015single}}          & \multicolumn{2}{c}{Manga109~\cite{matsui2017sketch}}                     \\ 
& \multirow{-2}{*}{}  & PSNR  & SSIM         & PSNR  & SSIM      & PSNR  & SSIM         & PSNR  & SSIM      & PSNR  & SSIM   \\ \midrule
Bicubic & \multirow{9}{*}{\tabincell{c}{x2}}  & 28.82 &0.8577   &26.02 &0.7634  &25.92 &0.7310	&23.14 &0.7258  &25.60 &0.8498  \\
CARN~\cite{ahn2018fast} & & 30.99 &0.8779	&28.10  &0.7879	   & 26.78 & 0.7286	    &25.27 &0.7630	    & 26.86 &0.8606  \\
Bicubic+ZSSR~\cite{shocher2018zero} & & 31.08 &0.8786	&28.35  &0.7933	   & 27.92 & 0.7632	    &25.25 &0.7618	    & 28.05 &0.8769  \\
Deblurring~\cite{pan2017deblurring}+CARN~\cite{shocher2018zero} & & 24.20 &0.7496	&21.12  &0.6170	   & 22.69 & 0.6471	    &18.89 &0.5895	    & 21.54 &0.7946  \\
CARN~\cite{shocher2018zero}+Deblurring~\cite{pan2017deblurring} & & 31.27 &0.8974	&29.03  &0.8267	   & 28.72 & 0.8033	    &25.62 &0.7981	    & 29.58 &0.9134  \\
IKC~\cite{gu2019blind} & & 37.19 &0.9526	&32.94  &0.9024	   & 31.51 & 0.8790	    &29.85 &0.8928	    & 36.93 &0.9667  \\
DANv1~\cite{luo2020unfolding} & & 37.34 &0.9526 	&33.08  &0.9041	   & 31.76 & 0.8858	    &30.60 &0.9060	    & 37.23 &0.9710  \\

DANv2~\cite{luo2021endtoend} &  & {\color[HTML]{3531FF} 37.60} & {\color[HTML]{3531FF} 0.9544}     & {\color[HTML]{3531FF} 33.44} & {\color[HTML]{3531FF} 0.9094}    & {\color[HTML]{3531FF} 32.00} & {\color[HTML]{3531FF} 0.8904}   & {\color[HTML]{3531FF} 31.43} & {\color[HTML]{3531FF} 0.9174}    & {\color[HTML]{3531FF} 38.07} & {\color[HTML]{3531FF} 0.9734}  \\ 

DCLS(Ours) &  & {\color[HTML]{FE0000} 37.63} & {\color[HTML]{FE0000} 0.9554}     & {\color[HTML]{FE0000} 33.46} & {\color[HTML]{FE0000} 0.9103}    & {\color[HTML]{FE0000} 32.04} & {\color[HTML]{FE0000} 0.8907}   & {\color[HTML]{FE0000} 31.69} & {\color[HTML]{FE0000} 0.9202}    & {\color[HTML]{FE0000} 38.31} & {\color[HTML]{FE0000} 0.9740}  \\

\midrule

Bicubic & \multirow{9}{*}{\tabincell{c}{x3}}  & 26.21 &0.7766   &24.01 &0.6662  &24.25 &0.6356	&21.39 &0.6203  &22.98 &0.7576  \\
CARN~\cite{ahn2018fast} & & 27.26 &0.7855	&25.06  &0.6676	   & 25.85 & 0.6566	    &22.67 &0.6323	    & 23.85 &0.7620  \\
Bicubic+ZSSR~\cite{shocher2018zero} & & 28.25 &0.7989	&26.15  &0.6942	   & 26.06 & 0.6633	    &23.26 &0.6534	    & 25.19 &0.7914  \\
Deblurring~\cite{pan2017deblurring}+CARN~\cite{shocher2018zero} & & 19.05 &0.5226	&17.61  &0.4558	   & 20.51 & 0.5331	    &16.72 &0.5895	    & 18.38 &0.6118  \\
CARN~\cite{shocher2018zero}+Deblurring~\cite{pan2017deblurring} & & 30.31 &0.8562	&27.57  &0.7531	   & 27.14 & 0.7152	    &24.45 &0.7241	    & 27.67 &0.8592  \\
IKC~\cite{gu2019blind} & & 33.06 &0.9146	&29.38  &0.8233	   & 28.53 & 0.7899	    &24.43 &0.8302	    & 32.43 &0.9316  \\
DANv1~\cite{luo2020unfolding} & & 34.04 &0.9199 	&30.09  &0.8287	   & 28.94 & 0.7919	    &27.65 &0.8352	    & 33.16 &0.9382  \\

DANv2~\cite{luo2021endtoend} &  & {\color[HTML]{3531FF} 34.12} & {\color[HTML]{3531FF} 0.9209}     & {\color[HTML]{3531FF} 30.20} & {\color[HTML]{3531FF} 0.8309}    & {\color[HTML]{3531FF} 29.03} & {\color[HTML]{3531FF} 0.7948}   & {\color[HTML]{3531FF} 27.83} & {\color[HTML]{3531FF} 0.8395}    & {\color[HTML]{3531FF} 33.28} & {\color[HTML]{3531FF} 0.9400}  \\ 

DCLS(Ours) &  & {\color[HTML]{FE0000} 34.21} & {\color[HTML]{FE0000} 0.9218}     & {\color[HTML]{FE0000} 30.29} & {\color[HTML]{FE0000} 0.8329}    & {\color[HTML]{FE0000} 29.07} & {\color[HTML]{FE0000} 0.7956}   & {\color[HTML]{FE0000} 28.03} & {\color[HTML]{FE0000} 0.8444}    & {\color[HTML]{FE0000} 33.54} & {\color[HTML]{FE0000} 0.9414}  \\

\midrule

Bicubic & \multirow{9}{*}{\tabincell{c}{x4}}  & 24.57 &0.7108   &22.79 &0.6032  &23.29 &0.5786	&20.35 &0.5532  &21.50 &0.6933  \\
CARN~\cite{ahn2018fast} & & 26.57 &0.7420	&24.62  &0.6226	   & 24.79 & 0.5963	    &22.17 &0.5865	    & 21.85 &0.6834  \\
Bicubic+ZSSR~\cite{shocher2018zero} & & 26.45 &0.7279	&24.78  &0.6268	   & 24.97 & 0.5989	    &22.11 &0.5805	    & 23.53 &0.7240  \\
Deblurring~\cite{pan2017deblurring}+CARN~\cite{shocher2018zero} & & 18.10 &0.4843	&16.59  &0.3994	   & 18.46 & 0.4481	    &15.47 &0.3872	    & 16.78 &0.5371  \\
CARN~\cite{shocher2018zero}+Deblurring~\cite{pan2017deblurring} & & 28.69 &0.8092	&26.40  &0.6926	   & 26.10 & 0.6528	    &23.46 &0.6597	    & 25.84 &0.8035  \\
IKC~\cite{gu2019blind} & & 31.67 &0.8829	&28.31  &0.7643	   & 27.37 & 0.7192	    &25.33 &0.7504	    & 28.91 &0.8782  \\
DANv1~\cite{luo2020unfolding} & & 31.89 &0.8864 	&28.42  &0.7687	   & 27.51 & 0.7248	    &25.86 &0.7721	    &{\color[HTML]{3531FF} 30.50} & {\color[HTML]{3531FF} 0.9037}  \\

DANv2~\cite{luo2021endtoend} &  & {\color[HTML]{3531FF} 32.00} & {\color[HTML]{3531FF} 0.8885}     & {\color[HTML]{3531FF} 28.50} & {\color[HTML]{3531FF} 0.7715}    & {\color[HTML]{3531FF} 27.56} & {\color[HTML]{3531FF} 0.7277}   & {\color[HTML]{3531FF} 25.94} & {\color[HTML]{3531FF} 0.7748}    & 30.45 & {\color[HTML]{3531FF} 0.9037}  \\ 

AdaTarget~\cite{jo2021adatarget}& & 31.58 &0.8814 	&28.14  &0.7626	   & 27.43 & 0.7216	    &25.72 &0.7683	    & 29.97 &0.8955  \\

DCLS(Ours) &  & {\color[HTML]{FE0000} 32.12} & {\color[HTML]{FE0000} 0.8890}     & {\color[HTML]{FE0000} 28.54} & {\color[HTML]{FE0000} 0.7728}    & {\color[HTML]{FE0000} 27.60} & {\color[HTML]{FE0000} 0.7285}   & {\color[HTML]{FE0000} 26.15} & {\color[HTML]{FE0000} 0.7809}    & {\color[HTML]{FE0000} 30.86} & {\color[HTML]{FE0000} 0.9086}  \\

\bottomrule
\end{tabular}
}
\caption{Quantitative comparison on datasets with \textit{Gaussian8} kernels. The best two results are marked in {\color{red}{red}} and {\color{blue}{blue}} colors, respectively.}
\label{table:iso_cmp}
\end{table*}


\begin{table*}[ht]
\setlength{\abovecaptionskip}{0.05in}
\setlength{\belowcaptionskip}{-0.05in}
\centering
\resizebox{0.91\linewidth}{!}{
\begin{tabular}{cccccccccccc}
\toprule
\multirow{2}{*}{Method $\times$4}& \multirow{2}{*}{Noise level} & \multicolumn{2}{c}{Set5~\cite{bevilacqua2012low}}              & \multicolumn{2}{c}{Set14~\cite{zeyde2010single}}     & \multicolumn{2}{c}{BSD100~\cite{martin2001database}}      & \multicolumn{2}{c}{Urban100~\cite{huang2015single}}          & \multicolumn{2}{c}{Manga109~\cite{matsui2017sketch}}                     \\ 
& \multirow{-2}{*}{}  & PSNR  & SSIM         & PSNR  & SSIM      & PSNR  & SSIM         & PSNR  & SSIM      & PSNR  & SSIM   \\ \midrule

Bicubic+ZSSR~\cite{shocher2018zero} &\multirow{5}{*}{\tabincell{c}{15}} & 23.32 &0.4868	&22.49  &0.4256	   & 22.61 & 0.3949	    &20.68 &0.3966	    & 22.04 &0.4952  \\
IKC~\cite{gu2019blind} & & 26.89 &0.7671	&25.28  &0.6483	   & 24.93 & 0.6019	    &22.94 &0.6362	    & 25.09 &0.7819  \\
DANv1~\cite{luo2020unfolding} & & 26.95 &0.7711 	&25.27  &0.6490	   & {\color[HTML]{3531FF} 24.95} & {\color[HTML]{3531FF} 0.6033}	    &23.00 &0.6407	    &25.29 & 0.7879  \\

DANv2~\cite{luo2021endtoend} &  & {\color[HTML]{3531FF} 26.97} & {\color[HTML]{3531FF} 0.7726}     & {\color[HTML]{3531FF} 25.29} & {\color[HTML]{3531FF} 0.6497}    & {\color[HTML]{3531FF} 24.95} & 0.6025   & {\color[HTML]{3531FF} 23.03} & {\color[HTML]{3531FF} 0.6429}    & {\color[HTML]{3531FF} 25.32} & {\color[HTML]{3531FF} 0.7896}  \\ 

DCLS(Ours) &  & {\color[HTML]{FE0000} 27.14} & {\color[HTML]{FE0000} 0.7775}     & {\color[HTML]{FE0000} 25.37} & {\color[HTML]{FE0000} 0.6516}    & {\color[HTML]{FE0000} 24.99} & {\color[HTML]{FE0000} 0.6043}   & {\color[HTML]{FE0000} 27.13} & {\color[HTML]{FE0000} 0.6500}    & {\color[HTML]{FE0000} 25.57} & {\color[HTML]{FE0000} 0.7969}  \\

\midrule

Bicubic+ZSSR~\cite{shocher2018zero} &\multirow{5}{*}{\tabincell{c}{30}} & 19.77 &0.2938	&19.36  &0.2534	   & 19.43 & 0.2308	    &18.32 &0.2450	    & 19.25 &0.3046  \\
IKC~\cite{gu2019blind} & & 25.27 &0.7154	&24.15  &0.6100	   & {\color[HTML]{3531FF} 24.06} & 0.5674	    &22.11 &0.5969	    & 23.80 &0.7438  \\
DANv1~\cite{luo2020unfolding} & & 25.32 & {\color[HTML]{3531FF} 0.7276} 	&24.15  & {\color[HTML]{3531FF}0.6138}	   & 24.04 & 0.5678	    &22.08 &0.5977	    &23.82 & 0.7442  \\

DANv2~\cite{luo2021endtoend} &  & {\color[HTML]{3531FF} 25.36} &  0.7264     & {\color[HTML]{3531FF} 24.16} & 0.6121    & {\color[HTML]{3531FF} 24.06} &  {\color[HTML]{3531FF} 0.5690}   & {\color[HTML]{3531FF} 22.14} & {\color[HTML]{3531FF} 0.6014}    & {\color[HTML]{3531FF} 23.87} & {\color[HTML]{3531FF} 0.7489}  \\ 

DCLS(Ours) &  & {\color[HTML]{FE0000} 25.49} & {\color[HTML]{FE0000} 0.7323}     & {\color[HTML]{FE0000} 24.23} & {\color[HTML]{FE0000} 0.6131}    & {\color[HTML]{FE0000} 24.09} & {\color[HTML]{FE0000} 0.5696}   & {\color[HTML]{FE0000} 22.37} & {\color[HTML]{FE0000} 0.6119}    & {\color[HTML]{FE0000} 24.21} & {\color[HTML]{FE0000} 0.7582}  \\


\bottomrule
\end{tabular}
}
\caption{Quantitative comparison on various noisy datasets. The best one marks in {\color{red}{red}} and the second best are in {\color{blue}{blue}}.}
\label{table:iso_noise_cmp}
\end{table*}



\subsection{Dual-Path Attention Network}

% To eliminate artifacts introduced from the DCLS and estimated kernels, we propose a dual-path attention network (DPAN) to reconstruct the high-quality HR image $\hat {\bf x}$. 
Unlike previous works~\cite{gu2019blind,luo2021endtoend} in which the dual-path structures are only used to concatenate the stretched kernel with blurred features, we propose to utilize primitive blur features as additive path to compensate the artifacts and errors introduced by the estimated kernel, known as dual-path attention network (DPAN).
% As shown in Fig.~\ref{fig:pipline}, 
DPAN is composed of several groups of dual-path attention blocks (DPAB), it receives both deblurred features $\widehat{\mathcal R}$ and primitive features ${\cal G}{\bf y}$. 
The right of Fig.~\ref{fig:pipline} illustrates the architecture of DPAB. 

Since the additive path of processing ${\cal G}{\bf y}$ is independently updated and used to concatenate with $\widehat{\mathcal R}$ to provide primary information to refine the deconvolved features. We can reduce its channels to accelerate training and inference, as the channel reduction (CR) operation illustrated in left of Fig.~\ref{fig:pipline}. Moreover, on the deconvolved feature path, we apply the channel attention layer~\cite{Zhang_2018_ECCV} after aggregating original features. In addition, we add a residual connection for each path on all groups and blocks. 
% Since the original features ${\cal G}{\bf y}$ are independently processed and are used to provide primary information to the deconvolved features, 
The pixelshuffle~\cite{huang2009multi} is used as the upscale module. We can jointly optimize the SR network and kernel estimation network as follows:
\begin{equation}
\centering
    {\cal L} =  l_1({\bf \hat k}, {\bf k}_l; \theta_k) + l_1({\bf \hat x}, {\bf x}; \theta_g)
\label{eq:loss}
\end{equation}
where $\theta_k$ and $\theta_g$ are the parameters of kernel estimation network and DCLS reconstruction network, respectively.

==> CVPR2022 - Super Resolution/related_work.tex <==
\section{Related work}

% \noindent \textbf{Single degradation SR}
\noindent \textbf{Non-blind SR}
% In the past few years, many works have employed deep CNNs to address the task of SISR due to their powerful feature representation capabilities. As a pioneer, deep learning based method is first proposed by SRCNN~\cite{dong2014learning} that maps LR images to HR ones by a convolutional network with three layers. Later, plenty of deep learning networks have been proposed for image super resolution~\cite{kim2016accurate,lim2017enhanced,ledig2017photo,zhang2017beyond,zhang2018image,shi2016real,lai2017deep,haris2018deep,kim2016deeply,tai2017image} achieving strong performance on bicubic downsampling images. Kim \textit{et al.}~\cite{kim2016accurate} introduced residual blocks into SR network. Lim \textit{et al.}~\cite{lim2017enhanced} removed the unnecessary batch normalization layer of network and proposed an enhanced deep SR(EDSR) network by taking advantage of the residual learning. Especially, Zhang \textit{et al.}~\cite{zhang2018residual} proposed RDN by utilizing residual dense blocks and further introduced the channel attention network(RCAN)~\cite{zhang2018image} for SR to achieve superior qualitative performance on PSNR. Although some SR methods have achieved good performance with respect to fidelity, the image of super-resolution have poor visual feeling with blurry or artifact. To address this issue, Wang \textit{et al.}~\cite{wang2018esrgan} proposed ESRGAN by utilizing adversarial losses and perceptual losses to improve the visual effects. Moreover, Wang \textit{et al.}~\cite{wang2018recovering} introduced feature transform layer based on segmentation prior to recover realistic texture in super-resolution image results.
Since pioneering work SRCNN~\cite{dong2014learning} proposes to learn image SR with a three-layer convolution network, most subsequent works have focused on optimizing the network architectures~\cite{kim2016accurate,lim2017enhanced,shi2016real,zhang2018residual,zhang2018image,lai2017deep,zhang2017beyond,haris2018deep,kim2016deeply,tai2017image,zhang2020residual,luo2021ebsr,dai2019second} and loss functions~\cite{ledig2017photo,wang2018esrgan,johnson2016perceptual,yu2016ultra,lugmayr2020srflow,zhang2018unreasonable,wang2018recovering}. These CNN-based methods have achieved impressive performance on SISR with a predefined single degradation setting (e.g., bicubic downsampling). However, they may suffer significant performance drops when the predefined degradation kernel is different from the real one. 

Some non-blind SR approaches address the multiple degradation problem by restoring HR images with given the corresponding kernels. Specifically, SRMD~\cite{zhang2018learning} is the first method that concatenates LR image with a stretched blur kernel as inputs to obtain a super-resolved image under different degradations. Later, Zhang \textit{et al.}~\cite{zhang2019deep,zhang2020deep} incorporate advanced deblurring algorithms and extend the degradation to arbitrary blur kernels. UDVD~\cite{xu2020unified} improves the performance by incorporating dynamic convolution. Hussein \textit{et al.}~\cite{hussein2020correction} introduce a correction filter that transfers blurry LR images to match the bicubicly designed SR model. Besides, zero-shot methods~\cite{xu2020unified,soh2020meta} have also been investigated in non-blind SR with multiple degradations.  

\noindent \textbf{Blind SR}
% Under the blind SR setting, HR image is recovered from LR image degraded with unknown kernel.
% In recent years, blind SR has attracted increasing attention to solve practical SR applications.
% Bell-Kligler \textit{et al.}~\cite{bell2019blind} proposed KernelGAN which estimates the degraded kernel by an internal generative adversarial network(GAN) on a single image. However, the accuracy of kernel estimation is limited due to the constraints of handcrafted is weakly. Based on KernelGAN, Liang \textit{et al.}~\cite{liang2021flow} proposed KernelGAN-FKP by utilizing a flow-based prior for kernel estimation. In addition, zero-shot learning have also been applied to blind SR. In ZSSR \textit{et al.}~\cite{shocher2018zero}, training is conducted at test time and an LR image as its input which can pay more attention to the internal information of the image. An inspiring work by Gu \textit{et al.}~\cite{gu2019blind} proposed IKC which uses a kernel prediction network with a correction network taking the current kernel prediction and SR result of the pre-trained SR model as input to correct the kernel estimation iteratively. However, it is time-consuming for applying a iterative framework. Luo \textit{et al.}~\cite{luo2020unfolding} proposed a deep alternating network (DAN) which consists of two modules restorer and estimator to form an end-to-end trainable network. Further more, Luo \textit{et al.}~\cite{luo2020unfolding} proposed DANv2 which estimates the kernel more accurately.
Under the blind SR setting, HR image is recovered from the LR image degraded with unknown kernel~\cite{levin2009understanding,levin2011efficient,michaeli2013nonparametric}. Most approaches solve this problem with a two stage framework: kernel estimation and kernel-based HR image restoration. For the former,  KernelGAN~\cite{bell2019blind} estimates the degradation kernel by utilizing an internal generative adversarial network(GAN) on a single image, and applies that kernel to a non-blind SR approach such as ZSSR to get the SR result. Liang \textit{et al.}~\cite{liang2021flow} improve the kernel estimating performance by introducing a flow-based prior. Furthermore, Tao \textit{et al.}~\cite{tao2021spectrum} propose a spectrum-to-kernel network and demonstrate that estimating blur kernel in the frequency domain is more conducive than in spatial domain. For the latter, Gu \textit{et al.}~\cite{gu2019blind} propose to apply spatial feature transform (SFT) and iterative kernel correction (IKC) strategy for accurate kernel estimation and SR refinement. Luo \textit{et al.}~\cite{luo2020unfolding} develop an end-to-end training deep alternating network (DAN) by estimating reduced kernel and restoring HR image iteratively. However, both IKC and DAN are time-consuming and computationally costly. The modified version of DAN~\cite{luo2021endtoend} conducts a dual-path conditional block (DPCB) and supervises the estimator on the complete blur kernel to further improve the performance.
